Adaptive Space-Time Beamforming in Radar Systems

The goal of this chapter is to review the recent work and advances in the area of space-time beamforming algorithms and their application to radar systems. These systems include phased-array \cite{melvin} and multi-input multi-output (MIMO) radar systems \cite{haimo_08}, mono-static and bi-static radar systems and other configurations \cite{melvin}. Furthermore, this chapter also describes in detail some of the most successful space-time beamforming algorithms that exploit low-rank and sparsity properties as well as the use of prior-knowledge to improve the performance of STAP algorithms in radar systems.

==> bibliography_mod.tex <==
\begin{thebibliography}{99}

\bibitem{klemm}
R. Klemm, Principle of space-time adaptive processing, IEE Press,
Bodmin, UK, 2002.

\bibitem{melvin}
W. L. Melvin, "A STAP overview", IEEE Aero. .Elec. Syst. Mag., vol.
19, no. 1, pp. 19–35, 2004.

\bibitem{brennan} L. E. Brennan and I. S.
Reed, "Theory of adaptive radar", IEEE Trans. Aero. Elec. Syst.,
vol. AES-9, no. 2, pp. 237–252, 1973.

\bibitem{reed}
I. S. Reed, J. D. Mallett, and L. E. Brennan, "Rapid convergence
rate in adaptive arrays", IEEE Trans. Aero. Elec. Syst., vol.
AES-10, no. 6, pp. 853–863, 1974.

\bibitem{kelly}
E. J. Kelly, "An adaptive detection algorithm", IEEE Trans. Aero.
Elec. Syst., vol. AES-22, no. 2, pp. 115–127, 1986.

\bibitem{haimovich}
A. M. Haimovich and Y. Bar-Ness, "An eigenanalysis interference
canceler", IEEE Trans. Sig. Process., vol. 39, no. 1, pp. 76–84,
1991.

\bibitem{robey}
F. C. Robey, D. R. Fuhrmann, E. J. Kelly, and R. Nitzberg, "A CFAR
adaptive matched filter detector", IEEE Trans. Aero. Elec. Syst.,
vol. 28, no. 1, pp. 208–216, Jan 1992.

\bibitem{ward}
J. Ward, "Space-time adaptive processing for airborne radar,", Tech.
Rep. 1015, MIT Lincoln lab., Lexington, MA, Dec. 1994.

\bibitem{haimovich_radar}
A. Haimovich, "The eigencanceler: adaptive radar by eigenanalysis
methods", IEEE Trans. Aero. Elec. Syst., vol. 32, no. 2, pp.
532–542, 1996.

\bibitem{goldstein}
J. S. Goldstein and I. S. Reed, "Reduced-rank adaptive filtering",
IEEE Trans. Sig. Process., vol. 45, no. 2, pp. 492–496, 1997.

\bibitem{goldstein2}
J. S. Goldstein and I. S. Reed, "Theory of partially adaptive
radar", IEEE Trans. Aero. Elec. Syst., vol. 33, no. 4, pp.
1309–1325, 1997.

\bibitem{gau}
Y.-L. Gau and I.S. Reed, "An improved reduced-rank CFAR space-time
adaptive radar detection algorithm", IEEE Trans. Sig. Process., vol.
46, no. 8, pp. 2139–2146, Aug 1998.

\bibitem{reed98}
I. S. Reed, Y. L. Gau, and T. K. Truong, "CFAR detection and
estimation for STAP radar", IEEE Trans. Aero. Elec. Syst., vol. 34,
no. 3, pp. 722– 735, 1998.

\bibitem{goldstein99}
J. S. Goldstein, I. S. Reed, and P. A. Zulch, "Multistage partially
adaptive STAP CFAR detection algorithm", IEEE Trans. Aero. Elec.
Syst., vol. 35, no. 2, pp. 645–661, 1999.

\bibitem{guerci}
J. R. Guerci, J. S. Goldstein, and I. S. Reed, "Optimal and adaptive
reduced-rank STAP", IEEE Trans. Aero. Elec. Syst., vol. 36, no. 2,
pp. 647–663, 2000.



\bibitem{haykin}
S. Haykin, Adaptive Filter Theory, NJ: Prentice-Hall, 4th, ed, 2002.

\bibitem{goldstein97}
J. S. Goldstein and I. S. Reed, "Subspace selection for partially
adaptive sensor array processing", IEEE Trans. Aero. Elec. Syst.,
vol. 33, no. 2, pp. 539–544, 1997.

\bibitem{goldstein98}
J. S. Goldstein, I. S. Reed, and L. L. Scharf, "A multistage
representation of the wiener filter based on orthogonal
projections", IEEE Trans. Inf. Theory, vol. 44, no. 7, pp.
2943–2959, 1998.

\bibitem{pados99}
D. A. Pados and S. N. Batalama, "Joint space-time auxiliary-vector
filtering for DS/CDMA systems with antenna arrays", IEEE Trans.
Commun., vol. 47, no. 9, pp. 1406–1415, 1999.

\bibitem{pados01}
D. A. Pados and G. N. Karystinos, "An iterative algorithm for the
computation of the MVDR filter", IEEE Trans. Sig. Process.], vol.
49, no. 2, pp. 290–300, Feb 2001.

\bibitem{pados07}
 D. A. Pados, G. N. Karystinos, S. N. Batalama, and J. D.
Matyjas, "Short-data-record adaptive detection", 2007 IEEE Radar
Conf., pp. 357– 361, 17-20 April 2007.

\bibitem{jdl}
H. Wang, and L. Cai, "On adaptive spatial-temporal processing for
airborne surveillance radar systems", IEEE Trans. Aero. Elec. Syst.,
vol. 30, no. 3, 660670, 1994.

\bibitem{adve1}
R. S. Adve, T. B. Hale, and M. C. Wicks, "Practical joint domain
localised adaptive processing in homogeneous and nonhomogeneous
environments. Part 1: Homogeneous environments.", IEE Proceedings
Radar, Sonar and Navigation, vol. 147, no. 2, 5765, 2000.

\bibitem{adve2}
R. S. Adve, T. B. Hale, and M. C. Wicks, "Practical joint domain
localised adaptive processing in homogeneous and nonhomogeneous
environments. Part 2: Nonhomogeneous environments.", IEE Proceedings
Radar, Sonar and Navigation, vol. 147, no. 2, 6674, 2000.

\bibitem{delamare_spl07}
R. C. de Lamare and R. Sampaio-Neto, "Reduced-rank adaptive
filtering based on joint iterative optimization of adaptive
filters", IEEE Sig. Proc. Lett., vol. 14, no. 12, pp. 980–983, 2007.

\bibitem{fa}
R. Fa, R. C. de Lamare, and D. Zanatta-Filho, "Reduced-rank STAP
algorithm for adaptive radar based on joint iterative optimization
of adaptive filters", in Conf. Record of the Fourty-Second Asilomar
Conf. Sig. Syst. Comp., 2008.

\bibitem{delamare_icassp07}
R. C. de Lamare and R. Sampaio-Neto, "Adaptive reduced-rank mmse
parameter estimation based on an adaptive diversity-combined
decimation and interpolation scheme", in Proc. IEEE Int. Conf.
Acous. Speech Sig. Process., 15–20 April 2007, vol. 3, pp.
III–1317–III–1320.

\bibitem{jidf}
R. C. de Lamare, and R. Sampaio-Neto, "Adaptive reduced-rank
processing based on joint and iterative interpolation, decimation,
and filtering", IEEE Trans. Sig. Process. , vol.57, no.7,
pp.2503-2514, July 2009

\bibitem{applebaum}
S. Applebaum and D. Chapman, "Adaptive arrays with main beam
constraints", IEEE Trans. on Ant. Prop., vol. 24, no. 5, pp.
650–662, 1976.

\bibitem{golub}
G. H. Golub and C. F. van Loan, Matrix Computations, Wiley, 2002.

\end{thebibliography}

